Lithium-rich giants in the Galactic thick disk

Context: Lithium is a fragile element, which is easily destroyed in the stellar interior. The existence of lithium-rich giants still represents a challenge for stellar evolution models. Aims: We have collected a large database of high-resolution stellar spectra of 824 candidate thick-disk giants having 2\,MASS photometry and proper motions measured by the Southern Proper-Motion Program (SPM). In order to investigate the nature of Li-rich giants, we searched this database for giants presenting a strong Li\,I resonance line. Methods: We performed a chemical abundance analysis on the selected stars with the MOOG code along with proper ATLAS-9 model atmospheres. The iron content and atmospheric parameters were fixed by using the equivalent width of a sample of Fe lines. We also derive abundances for C, N, and O and measure or derive lower limits on the $^{12}$C/$^{13}$C isotopic ratios, which is a sensible diagnostic of the stars evolutionary status. Results: We detected five stars with a lithium abundance higher than 1.5, i.e. Li-rich according to the current definition. One of them (SPM-313132) has A(Li)$>$3.3 and, because of this, belongs to the group of the rare super Li-rich giants. Its kinematics makes it a likely thin-disk member and its atmospheric parameters are compatible with it being a 4\,M$_\odot$ star either on the red giant branch (RGB) or the early asymptotic giant branch. This object is the first super Li-rich giant detected at this phase. The other four are likely low-mass thick-disk stars evolved past the RGB luminosity bump, as determined from their metallicities and atmospheric parameters. The most evolved of them lies close to the RGB-tip. It has A(Li)$>$2.7 and a low $^{12}$C/$^{13}$C isotopic ratio, close to the cool bottom processing predictions.

==> distance.tex <==
\begin{table*}
\caption{Derived distances and orbital parameters of the program stars.}
\label{dist}
\begin{center}
\tiny
\begin{tabular}{lccccccrrrrr}
\hline
 SPM    &   R$_\odot$  &    X	  &   Y   &  Z        &   U	  &	 V   &    W    & e  &  Z$_{max}$ & R$_{p}$ & R$_{a}$	  \\
       &   kpc       & kpc	  & kpc   &  kpc      &  \kms	  &\kms      &   \kms  &    &  kpc    &   kpc & kpc  \\ 
\hline
142173 &  3.6$\pm$0.3	 & 7.91  &  -0.50  & -3.50   & 195$\pm$36 &  -41$\pm$39 & 36$\pm$9 & 0.90$\pm$0.09 & 8.23$\pm$0.49& 0.54$\pm$0.03&  10.10$\pm$0.53\\ 
171877 &  3.1$\pm$0.3	 & 8.25  &  -0.13  & -3.13   & -17$\pm$28 &   82$\pm$37 & 27$\pm$3 & 0.61$\pm$0.01 & 2.19$\pm$0.06& 1.97$\pm$0.01&   8.20$\pm$0.02\\ 
225245 &  7.3$\pm$0.7	 & 8.55  &  -0.10  & -7.28   & -56$\pm$41 &   52$\pm$43 &  6$\pm$1 & 0.71$\pm$0.04 & 5.40$\pm$0.19& 1.44$\pm$0.02&   8.68$\pm$0.23\\ 
313132 &  0.7$\pm$0.1	 & 8.51  &  -0.11  & -0.70   & -50$\pm$11 &  165$\pm$11 & 12$\pm$2 & 0.29$\pm$0.01 & 0.63$\pm$0.01& 5.00$\pm$0.01&   9.00$\pm$0.01\\ 
343555 &  1.1$\pm$0.1	 & 8.60  &  -0.14  & -1.07   & -33$\pm$ 9 &   29$\pm$20 &-84$\pm$3 & 0.85$\pm$0.02 & 2.19$\pm$0.11& 0.73$\pm$0.02&   8.89$\pm$0.12\\ 
\hline
\end{tabular}
\end{center}
\end{table*}				  

